Meta-Learning Online Adaptation of Language Models

Large language models encode impressively broad world knowledge in their parameters. However, the knowledge in static language models falls out of date, limiting the model's effective "shelf life." While online fine-tuning can reduce this degradation, we find that naively fine-tuning on a stream of documents leads to a low level of information uptake. We hypothesize that online fine-tuning does not sufficiently attend to important information. That is, the gradient signal from important tokens representing factual information is drowned out by the gradient from inherently noisy tokens, suggesting that a dynamic, context-aware learning rate may be beneficial. We therefore propose learning which tokens to upweight. We meta-train a small, autoregressive model to reweight the language modeling loss for each token during online fine-tuning, with the objective of maximizing the out-of-date base question-answering model's ability to answer questions about a document after a single weighted gradient step. We call this approach Context-aware Meta-learned Loss Scaling (CaMeLS). Across three different distributions of documents, our experiments find that CaMeLS provides substantially improved information uptake on streams of thousands of documents compared with standard fine-tuning and baseline heuristics for reweighting token losses.

==> history/abs.tex <==
LLMs are useful but fall out of date

Online fine-tuning can help, but there's a massive amount of data and fine-tuning on all of it is challenging and costly.

Further, our experiments show that fine-tuning an LM on a stream of news documents leads to very low information uptake.

We hypothesize that to maximize knowledge uptake in online fine-tuning, the loss for some tokens is more informative about the state of the world than others, and the learning rate should therefore be dynamically updated.

Leveraging this hypothesis, we meta-train a small, autoregressive model to reweight the language modeling loss at each timestep for an out-of-date base language model, maximizing the base LM's ability to answer questions about a document after a single weighted gradient step.

We find that fine-tuning on a stream of thousands of documents with the meta-learned importance weights increases knowledge retention by 3x compared to standard online fine-tuning.

Further, we find that the meta-learned weights are general, and a single reweighting model can be used to enhance the online adaptation of any LM.

